The Trusted Computing Base of the CompCert Verified Compiler

CompCert is the first realistic formally verified compiler: it provides a machine-checked mathematical proof that the code it generates matches the source code. Yet, there could be loopholes in this approach. We comprehensively analyze aspects of CompCert where errors could lead to incorrect code being generated. Possible issues range from the modeling of the source and the target languages to some techniques used to call external algorithms from within the compiler.

==> TCB_table.tex <==
\begin{figure}[ht]
\centering
\begin{tabular}{c@{~}|@{~}c@{~}|@{~}c}
TCB part & Bugs in the generated code & See \\\hline
\coq\ kernel & Highly unlikely & \S~\ref{sec:CoqKernel}\\
\coq\ extraction & Very unlikely & \S~\ref{sec:extraction}\\
Unsound \coq\ model of \ocaml\ oracles & Unlikely (modulo careful review) & \S~\ref{sec:mismatch}\\
Other incorrect \coq\ axiom & Idem & \S~\ref{sec:logicalcontradiction}\\
C formal syntax/semantics (Front-end) & Happened in very rare cases & \S~\ref{sec:frontend}\\
Pretty-printing of assembly & Idem & \S~\ref{sec:prettyprint}\\
Model of the ABI & Idem & \S~\ref{sec:ABI}\\
Pseudo-instructions (Spec. vs Implem.) & Happened in not so rare cases & \S~\ref{sec:pseudoinst}\\
\end{tabular}
\caption{Informal classification of the risk for \CompCert\ to generate incorrect code, by subpart of the TCB (from our experience).\label{fig:TCB}} 
\end{figure}

